Robust-Locomotion-by-Logic: Perturbation-Resilient Bipedal Locomotion via Signal Temporal Logic Guided Model Predictive Control

This study introduces a robust planning framework that utilizes a model predictive control (MPC) approach, enhanced by incorporating signal temporal logic (STL) specifications. This marks the first-ever study to apply STL-guided trajectory optimization for bipedal locomotion, specifically designed to handle both translational and orientational perturbations. Existing recovery strategies often struggle with reasoning complex task logic and evaluating locomotion robustness systematically, making them susceptible to failures caused by inappropriate recovery strategies or lack of robustness. To address these issues, we design an analytical stability metric for bipedal locomotion and quantify this metric using STL specifications, which guide the generation of recovery trajectories to achieve maximum robustness degree. To enable safe and computational-efficient crossed-leg maneuver, we design data-driven self-leg-collision constraints that are $1000$ times faster than the traditional inverse-kinematics-based approach. Our framework outperforms a state-of-the-art locomotion controller, a standard MPC without STL, and a linear-temporal-logic-based planner in a high-fidelity dynamic simulation, especially in scenarios involving crossed-leg maneuvers. Additionally, the Cassie bipedal robot achieves robust performance under horizontal and orientational perturbations such as those observed in ship motions. These environments are validated in simulations and deployed on hardware. Furthermore, our proposed method demonstrates versatility on stepping stones and terrain-agnostic features on inclined terrains.

==> active_toe.tex <==


Active toe joint is popular among quasi-static bipedal robots; the joint regulates the upper body balance \cite{active_toe_mexico} and achieve faster walking \cite{active_toe_enhance}. However, it is less adopted by the dynamic walking bipeds such as Cassie \cite{gong2018feedback, HLIP_TRO_XIONG}. The authors in \cite{shamsah2023TRO} actuated the toe to improve the velocity tracking. 



==> archive.tex <==
\subsection{Keyframe-based Non-periodic Locomotion} \label{keyframe_loco}

\begin{defn}[Locomotion keyframe]\label{def:STL_keyframe}
A keyframe $\mathcal{K}$ is defined as a system state at apex time---the time when CoM passes over the stance foot in the sagittal direction. The keyframe is composed of CoM position $p(t) = [x(t), y(t)]^T$ and velocity $\dot{p}(t)$ in both sagittal and lateral directions. $\mathcal{K}_X = [p, \dot{p}]$.
\end{defn}

To define a multi-step walking motion for bipedal robot walking, we separate the entire trajectory into multiple OWS phases that start and end at a keyframe state \cite{Zhao2017IJRR}. The $i^{th}$ OWS cycle can be represented by a discrete keyframe transition pair $(k^i, k^{i+1})$. The keyframe contains the sagittal and lateral CoM apex state, as well as the stance foot index (Sec. \ref{LTL_spec}). Given two consecutive keyframe states in the sagittal plane, forward and backward numerical integration is used to solve for the contact switching time of OWS. The lateral keyframe transition is determined once the time ($t_1$ and $t_2$ for the first-half and second-half OWS phases, respectively) is found, which gives the CoM state $(p_{\rm switch},\dot{p}_{\rm switch})$ at contact switch instant. The next foot placement can be computed in the lateral direction from the current keyframe with the analytical solution: 

\begin{equation}
\begin{aligned}
p_{\rm foot} = p_{\rm switch} + \frac{(e^{2\omega_{\rm asym} t_2}-1)\dot{p}_{\rm switch}}{(e^{2\omega_{\rm asym} t_2}+1)\omega_{\rm asym}}
\label{eq:anal_keys}
\end{aligned}
\end{equation}
where the asymptote slope $\omega_{\rm asym} = \sqrt{g/h_{\rm apex}}$ and $h_{\rm apex}$ is the relative apex CoM height with respect to the stance foot height. $g$ is the gravity constant. Detailed derivations can be referred in the work of \cite{Zhao2017IJRR}.


Compared to periodic walking, where the robot repeats the same motion pattern periodically, keyframe-based walking allows for non-periodic walking that better accommodates rough terrain and environment disturbances. A keyframe decision maker is thus necessary to design safe and feasible keyframe transitions at runtime.


\section{Signal Temporal Logic}

Signal temporal logic (STL) \cite{STL_Origin}  use logical symbols of negation ($\neg$), disjunction ($\vee$), and conjunction ($\wedge$). Temporal operators such as ``eventually" ($\Diamond$), ``always" ($\square$), and until ($\mathcal{U}$) are used. The specification formulas are defined with the following syntax:
\begin{equation}\begin{split}
\varphi ::= 
& \mu^\pi \;|\; \neg\varphi \;|\; \varphi_1 \wedge \varphi_2 \;|\; \varphi_1 \vee \varphi_2 \;|\; \\ 
& \Diamond_{[a,b]}\;\varphi \;|\; \square_{[a,b]}\;\varphi \;|\; 
\varphi_1 \; \mathcal{U}_{[a,b]}\; \varphi_2 \;|\; \varphi_1 \;\mathcal{E}_{[a,b]}\; \varphi_2
\end{split}\end{equation}
where $\varphi$, $\varphi_1$, and $\varphi_2$ are STL formulas. $\mu^\pi$ is a predicate defined by a vector-valued function $\mu^\pi(y): \mathcal{R}^p \to \mathcal{R}$ of the signal $y$. $0 \leq a \leq b < \infty$ denote time intervals. The symbol $\Diamond$ represents \textit{eventually}, and $\square$ represents \textit{always}. The $\mathcal{U}$ denotes \textit{until}, and the $\mathcal{E}$ denotes \textit{except}, which means $\varphi_2$ is satisfied only once during $[a,b]$, and $\varphi_1$ is satisfied at all other times. This requires that $\varphi_1$ and $\varphi_2$ cannot be both satisfied at the same time. We will use this syntax to represent the semantics that an event happens once and only once during a time window. A signal $y = y_0y_1y_2...$ satisfies $\varphi$ is denoted by $y \models \varphi$.

STL provides a unique benefit of admitting \textit{quantitative semantics}, which denotes the notion of \textit{robustness degree} \cite{MTL_Papas}. In addition to the boolean satisfaction metric, STL allows the maximization of the margin of robustness. In a dynamic environment, where the system must react to new unforeseen events such as impacts, it is useful to have a margin of maneuverability to react without violating the formula \cite{fly-by-logic}. The quantitative semantics can also lead to a minimally violating trajectory if the formula cannot be satisfied. Tab.\ref{tab:robustness} shows the signal temporal logic robustness semantics. 
\begin{table}[H]
\centering
TABLE I \\
SEMANTICS OF SIGNAL TEMPORAL LOGIC ROBUSTNESS
\begin{tabular}{c c c} \\ 
\hline

$y =\varphi$ &  $\Leftrightarrow$ & $\rho ^ \varphi((y,0))$   \\ 
$\rho ^ \pi ((y,t))$ & $\Leftrightarrow$ & $\mu ^ \pi  (y_t) - c$ \\
$\rho ^ {\neg\varphi} ((y,t))$ & $\Leftrightarrow$ & $-\rho ^ \varphi  ((y,t))$ \\
$\rho ^ {\varphi_1 \land \varphi_2} ((y,t))$ & $\Leftrightarrow$ & min$(\rho ^ {\varphi_1} ((y,t)),\rho ^ {\varphi_2} ((y,t)))$ \\
$\rho ^ {F_{[t_1,t_2]}\varphi}((y,t))$ & $\Leftrightarrow$ & max$_{t^{'}\in[t+t_1,t+t_2]} (\rho^{\varphi} ((y,t^{'})))$ \\
$\rho ^ {G_{[t_1,t_2]}\varphi}((y,t))$ & $\Leftrightarrow$ & min$_{t^{'}\in[t+t_1,t+t_2]} (\rho^{\varphi} ((y,t^{'})))$\\
$\rho ^ {{\varphi_1}U_{[t_1,t_2]}{\varphi_2}} ((y,t))$ & $\Leftrightarrow$ & \makecell{max$_{t^{'}\in[t+t_1,t+t_2]}($min$([\rho^{\varphi_{1}}((y,t^{'})),$\\min $_{t^{''}\in[t+t_1,t^{'}]}(\rho^{\varphi_{2}}((y,t^{''})))]^T))$} \\ 
 
\hline
\end{tabular}
\end{table}
\label{tab:robustness}

\section{Bi-level Optimization with Mixed Integer Programming and Trajectory Optimization}


The bilevel optimization formulation is a two layer optimization with the top layer has variables equal to the output of the bottom layer.

\subsection{Collision-Aware Kinodynamic Trajectory Optimization}
\label{TO_implement}
% Why TO.
The task planner and PABTs generate keyframe transitions robust to perturbations. However, mapping the transitions to whole-body trajectories in real-time often poses a challenge due to the curse of dimensionality. To address this, we use TO to create a set of motion primitives offline. The TO generates desired motions that satisfy the physical constraints while minimizing the trajectory cost \cite{RaoOptimalControl, Frost, RT_collision}. The TO is also used as a verification to check the feasibility of high-level keyframe transitions.
%Our TO methods incorporates self-collision and keyframe boundary constraints to ensure that the optimal full-body motion is collision-free and obeys high-level keyframe decisions.
The nonlinear program (NLP) of TO is formulated as:

\begin{align}
%\begin{aligned}
\label{eq:optimization}
\argmin_{X} \quad  & \sum_{j=1}^{D}  \sum_{i=0}^{N_j} \Omega_j \cdot \mathcal{L}_j(x^j_i, u^j_i) \\\nonumber
\textrm{s.t.} \quad & H_j(x^j_i) \dot{x}_i + V_j(x^j_i) + G_j(x^j_i) = u_i, \quad (\textnormal{dynamics})  \\\nonumber
                & x_{0}^{j+1} = \Delta_j(x_{N_j}^j),  \qquad\qquad\qquad\qquad\,\, (\textnormal{reset\,map}) \\\nonumber
                 & \lambda_{c,z}\geq 0,  \; |\lambda_{c,xy}| \leq \mu \lambda_{c,z}, \qquad\qquad\quad\;\;\,  (\textnormal{friction}) \\\nonumber
                & C_j^{\rm kin}(x^j_i) \leq 0, \qquad\qquad\qquad\qquad\quad\,\,(\textnormal{kinematics})  \\\nonumber
                & \rm{Pr}(C_j^{\rm col}(x^j_i) \leq 0) \geq \emph{p}_x, \qquad\qquad\quad\qquad\;\;\;\;\;\, (\textnormal{self-collision}) \\\nonumber
                & C_j^{\rm key}(x^j_i, u^j_i) = 0  \qquad\qquad\;\;\; (\textnormal{keyframe\;boundary})
%\end{aligned}
\end{align}
\noindent where the domains include $D=2$ continuous single stance phases and 1 velocity reset map. Each single stance contains $N_j$ nodes, which represents a state-control pair $n^j_i=(x^j_i, u^j_i)$ at the $i^{\rm th}$ instant; the state represents the $x = [q;\dot{q}]$ with $q$ denoting the robot generalized coordinate states.
The NLP above solves the optimal state-control trajectory $X^* = \{n^{j*}_i\}$ by minimizing the pseudo energy $\mathcal{L}(\cdot) = || u_i ||^2$ with weights $\Omega_j$ while enforcing the physical constraints of the robot.  

The physical constraints shape the resultant trajectory.
The dynamics constraint is enforced between node points using Hermite-Simpson collocation. $H$, $V$, and $G$ denote the inertia, coriolis, and gravity matrices of the robot's rigid body dynamics.
$x_{0}^{j+1} = \Delta_j(x_{N_j}^j)$ maps the velocity jump between two consecutive stance modes. The horizontal contact forces $\lambda_{c,xy}$ are bounded by a linearized friction cone. 
The kinematics constraints $C_j^{\rm kin}(x^j_i)$ ensure that the joint angles, foot positions, and CoM trajectories are bounded.
$M$ geometric point pairs $(\bm{g}^m_l, \bm{g}^m_r)$ on two legs are selected as self-collision constraints (see Fig.~\ref{fig:framework}d). The signed distances are evaluated at each geometric point pair using forward kinematics $FK_{\bm{g}^m}(x_i)$ for all $m \in M$, $i \in N_j$.
%
\begin{equation}
\begin{aligned}
\bm{d}^m(x_i) &= FK_{\bm{g}^m_l}(x_i) - FK_{\bm{g}^m_r}(x_i), \\
C_j^{\rm col}(x_i) &= ||\bm{d}^m_{\rm min}||_2^2 - ||\bm{d}^m(x_i)||_2^2.
\label{eq:col_constr}
\end{aligned}
\end{equation}
% Because cassie's foot is narrow, the linear complementary constraints ensure that the stance foot has a line contact with the ground, which has 1 degree-of-freedom.
% We use phase space planning to find the next lateral keyframe.
The keyframe transition $(k^c, k^n)$ commanded from the task planner is enforced as a boundary condition for the foot placement, the apex CoM position and velocity. 

\subsection{Trajectory Optimization Integration with Mixed Integer Programming}

In this section, we talk about the connection between the trajectory optimization and mixed integer programming. This combination are heurachical and place a connection between offline generated trajectory and online gait selection using MIP.

%Assuming we have $\mathcal{K}$ time instances in the dynamic time window. We introduce the contact selection variable $s_k$ to indicate the contact state at each instance. $s_k$ is binary: $s_k = 1$ at contact instant, and $s_k = 0$ otherwise. Because the encoding introduces the binary variable $s_k$, we use this feature to introduce the new specification that denote a certain event happens once and only once. This means to the sum of the binary variables equal to 1. So we get constraints of $\Sigma s_k = 1, k \in \mathcal{K}$, to enforce that only one contact happening in the expected contact windows $\mathcal{K}$. This is effectively to enforce that the control $u = p\_{st \to sw}$ only applies to the system at contact time. It reset the CoM state from the final state of the current step to the initial state of the next step. For other instances, the control $u$ does not change the system dynamics, and the CoM state evolves based exclusively on the state update.

%The MILP will find the proper contact time similar to the phase-based trajectory optimization \cite{Winkler_towr}.
%The time slice cannot capture the exact instant when apex state occurs (i.e., lowest sagittal velocity) because the time axis is discretized. 
%We define the apex instant to be the time slice when the position of CoM surpass the foothold in the sagittal axis. The apex state is specified by STL to stay within the Riemannian partitions $\mathcal{R}$: $$\square(A_i Z_i) \models \pi^{\mathcal{R}_i}$$ where $\mathcal{R}_i$ is the Riemannian partition of the $i$th step in the dynamic-window. $Z_i$ is a vector indicates the cell number of the CoM state $A_i$. These specification and the discretized LIP model would together determine the location of the foot placements for the next two steps. The foot placements are fixed values during OWS and change only at contact events.

\subsection{motivation for not using Horizon Design I}
\label{horizon1}
We argue that one step horizon is not enough for foot placement calculation in the low level control. Assuming the reactive synthesis has only one step horizon, the next keyframe state is generated at every apex time. In this case, the robot only have $T/2$ until it reaches the contact time. In nominal walking, that's about 0.2s. This causes two problems.
During the first $T/2$ before the apex time, the foot placement calculation requires a desired keyframe after the contact, which is not available in one-step horizon. So it doesn't have a foot placement to target, which prevent the calculation of the swing foot trajectory. 
The second $T/2$ have a sharp change of foot location after the keyframe decisions are made. This can lead to a jerky motion for swing leg and possibly ruin the robot stability. 

Based on the issue of one-step horizon, we plan two steps ahead, i.e. to solve two next keyframes decisions from the current keyframe time ($H = 2$). The keyframe planning is apex-to-apex style. The reactive synthesis gives us a control sequence for keyframe transitions. New command are generated at every apex time. At contact time, we can calculate the swing foot location for next contact, and we can design a smooth trajectory toward that contact location.
We have a specification to ensure the target apex velocity is available after two future contacts. This is equivalent to set a MPC horizon of at least two apex steps. 

The total time $T_i$ is encoded as the $i^{\rm th}$ apex-to-apex step. We have environment information as signals. 

%The problem of horizon design I in \ref{horizon1} is that it requires a dynamics equation between apex to apex because the states are defined only at keyframe times. The apex to apex dynamics for LIP is not linear, thus making the MIP nonlinear. This causes numerical issue for branch-and-bound algorithm. To circumvent this, we propose to use a new horizon design which we call the flexible phasing MILP as shwon in Fig.~\ref{fig:horizon2}. This design allows non-fixed time and linear dynamics, so it make the problem feasible. However, it would introduce more state variables and thus make this problem harder to solve.

% Talk about the selection of discrete dynamics than s2s dynamics.
%Traditional horizon design \cite{HLIP_TRO_XIONG, } requires step-to-step dynamics because the states are not defined during the swing phase. However, the apex-to-apex dynamics is not linear, making any optimization formulation using this dynamics nonlinear too. This causes a numerical issue for the MIP solvers that uses branch-and-bound algorithm, which affects the solution quality and solving speed. To circumvent the issue, we propose to use a new horizon design which we call the dynamic-window horizon as shown in Fig.~\ref{fig:timeline}. This design adopt a non-fixed time window as the horizon, making it possible to use linear dynamics. It would, however, introduce more state variables and make this problem more complex.

% In this study, we propose a novel dynamic-window horizon, as depicted in Fig.~\ref{fig:horizon2}. The time axis is partitioned into short intervals, $\delta t$, chosen based on a trade-off between model accuracy and problem scale. %Larger values of $\delta t$ result in a less precise model approximation, while smaller values significantly increase the number of states. The signal $\boldsymbol{\bar{y}}_i$ at $t_i = i\delta t, i \in \mathcal{Z}$ time instances are modeled as discrete-time decision variables, and the resulting dynamics are linear, as demonstrated in Sec.\ref{sec:dynamics}.

% And between these fixed intervals, the dynamics is linear and can be interpreted as LIP model:
% $$X_{k+1} = A_d \cdot X_{k} + B_d \cdot s_k \cdot u$$
% where $A_d := exp(A \delta t)$ and $B_d = [0_{2\times2} \; I_{2\times2}]^T$ are the discretized state space value of LIP. The state $X_k = [x\;y\;dx\;dy]_k^T$ is the CoM position in stance foot frame. 


\section{one-step keyframe angular momentum based foot placement}

This section talks about the continuous foot placement calculation at 2k Hz based on angular momentum. We incorporated the momentum-based footstep planning and control architecture from \ref{}. We use the Linear Inverted Pendulum Model. However, instead of choosing normal velocity as state, we use angular momentum around contact foot as part of the system state. The reason is .... (from yukai's paper) \cite{MomentumController}\cite{PassivityControl}.

Momentum about the contact point is defined by the position of the foot and the centroidal dynamics. Even in the context of an aerial phase, we can use desired momentum states to regulate landing.

\begin{equation}
\begin{aligned}
L=L_{CoM}+ \textbf{p} \times m\textbf{v}_{CoM}
\end{aligned}
\end{equation}

Using LIPM, we assume the GRF is along the leg stick, which means GRF cannot generate force moment on the system, and we can never achieve back flip motion using the LIP model.
But using centroidal momentum model, we introduce more variables to the state and control, making the system dynamics more complicated.

The contact momentum is not zero but close. That's why we need detailed reactive planning from phase space. 

% This is the normal state space equation.
% \begin{equation}
% \begin{aligned}
% \centering
% \begin{bmatrix}
% \dot{x} \\
% \ddot{x} 
% \end{bmatrix}
% =
% \begin{bmatrix}
% 0 & 1 \\
% g/H & 0
% \end{bmatrix}
% \begin{bmatrix}
% x \\
% \dot{x}
% \end{bmatrix}
% \label{eq:LIMP}
% \end{aligned}
% \end{equation}

\begin{equation}
\begin{aligned}
\centering
\begin{bmatrix}
\dot{x} \\
\dot{L^y} 
\end{bmatrix}
=
\begin{bmatrix}
0 & 1/mH \\
mg & 0
\end{bmatrix}
\begin{bmatrix}
x \\
L^y
\end{bmatrix}
\label{eq:LIMP_momentum}
\end{aligned}
\end{equation}

From the current state, we can predict the future state at time $\tilde{t}$ before foot contact switch.
% This is the normal state prediction.
% \begin{equation}
% \begin{aligned}
% \centering
% \begin{bmatrix}
% x(\tilde{t}) \\
% \dot{x}(\tilde{t}) 
% \end{bmatrix}
% =
% \begin{bmatrix}
% cosh(l(\tilde{t}-t))  & sinh(l(\tilde{t}-t))/l \\
% l sinh(l(\tilde{t}-t))& cosh(l(\tilde{t}-t))
% \end{bmatrix}
% \begin{bmatrix}
% x(t) \\
% \dot{x}(t)
% \end{bmatrix}
% \label{eq:state_predict}
% \end{aligned}
% \end{equation}

\begin{equation}
\begin{aligned}
\centering
\begin{bmatrix}
x(\tilde{t}) \\
L^y(\tilde{t}) 
\end{bmatrix}
=
\begin{bmatrix}
cosh(\omega ((\tilde{t}-t)) & \frac{1}{mH\omega}sinh(\omega((\tilde{t}-t)) \\
mH \omega sinh(\omega ((\tilde{t}-t)) & cosh(\omega((\tilde{t}-t))
\end{bmatrix}
\begin{bmatrix}
x(t) \\
L^y(t) 
\end{bmatrix}
\label{eq:L_next}
\end{aligned}
\end{equation}

where $\omega=\sqrt{g/H}$, $t$ is the current time and $t \leq \tilde{t} \leq T$, and $T$ is the expect switch contact time. 
Then we could use this prediction to plan/adjust our foot placement $p_{sw}$. 
% \begin{equation}
% \begin{aligned}
% L^y(t_1) &= mHlsinh(w((t_1-t)) x(t) + cosh(w((t_1-t)) L^y(t)\\
% L^{yd}(t_2) &= mHlsinh(w((t_2)) p_{st} + cosh(w((t_2)) L^y(t_1)
% \end{aligned}
% \end{equation}

\section{LTL actions}

The system takes actions $a_{\rm sys} \in \mathcal{A}_{\rm sys} \subseteq \mathcal{R}_{s} \cup \mathcal{R}_{l} \cup \mathcal{L} \cup \mathcal{W}$ to decide the next keyframe state $k^n$. $\mathcal{L} = \{\textsf{small}, \textsf{medium}, \textsf{large}\}$ and $\mathcal{W} = \{\textsf{small}, \textsf{medium}, \textsf{large}\}$ represent the step length and width. $l \in \mathcal{L}$ and $w \in \mathcal{W}$ are the distances between the current and the next foot placements projected on sagittal and lateral axis. Note that $\mathcal{R}_{s}, \mathcal{R}_{l}$ are the relative CoM apex state in foot frame while $\mathcal{L}, \mathcal{W}$ are the global distances between footholds. Together, they completely define a transition action.

The environment state is represented by a perturbation set $p_{\rm env} \in \mathcal{P}_{\rm env} \coloneqq \mathcal{R}_{s} \cup \mathcal{R}_{l} \cup \{ \emptyset\}$ that pushes the system to a specific Riemannian cell center. In the task planner, we assume that the environment action is a perturbation only applied at a keyframe instant. The perturbation induces a CoM position and velocity jump after applying an external force to the robot's pelvis frame. The environment can also choose to not perturb, i.e., $p_{\rm env} = \emptyset$. The system action $\mathcal{A}_{\rm sys}$ and environment action $\mathcal{P}_{\rm env}$ together decides the next apex keyframe state $k^{n} = \mathcal{T}_{\rm SE}(k^c, a_{\rm sys}, p_{\rm env})$. Both actions are a part of the automaton state $\mathcal{S}$.

\section{Momentum Footstep Adjustment}
\label{Sec:angular_momentum_controller}
At the end of the next step, the angular momentum is estimated by
\begin{equation}
\begin{aligned}
\centering
L^y(T^-_{k+1},t)=mH \omega sinh(\omega T)x_c(T_k^+)+cosh(\omega T)L^y(T_k^+,t)
\label{eq:L_next}
\end{aligned}
\end{equation}
The angular momentum about the next contact point will be equal to the angular momentum about the current stance leg. However this is only true if the CoM height is constant and the ground is flat. 
\begin{equation}
\begin{aligned}
\centering
L^y(T^+_{k+1},t)=L^{y,d}(T^-_{k+1},t)
\label{eq:L_predic}
\end{aligned}
\end{equation}

The longitudinal target step position can thus be calculated using the following closed form solution
\begin{equation}
\begin{aligned}
\centering
p^{x,d}_{sw}(T^-_k)=\dfrac{L^{y,d}(T^-_{k+1})-cosh(\omega T)L^y(T_k^-,t)}{mH \omega sinh(\omega T)}
\label{eq:footstep}
\end{aligned}
\end{equation}

Since angular momentum about the contact point is decoupled between the x,y-axes, the lateral control can be assumed to be identical to longitudinal foot placement control. 

However, the angular momentum of the next walking step $L^{x,d}(T^-_{k+1})$ must be known in order to plan footsteps with a non-zero lateral stance width. Assuming an average zero velocity, a simple periodically oscillating LIP model can be sufficient to obtain $L^{x,d}$

\begin{equation}
\begin{aligned}
\centering
L^{x,d}(T^-_{k+1})=\frac{1}{2}mHW\frac{\omega sinh(\omega T)}{1+cosh(\omega T)}
\label{eq:footstep}
\end{aligned}
\end{equation}
where W is the desired step width. Note that $L$ is $+$ or $-$ depending on the stance leg. Turning is then commanded by assuming a target direction and calculating $L^{y,d}$ and $L^{x,d}$ in the new desired frame. 

Note that when Cassie is walking faster than 1 m/s, the vertical velocity $v^z_{com}$ can no longer be assumed to be zero. Faster speeds thus need to modify the above equation with the more general momentum equation

\begin{equation}
\begin{aligned}
\centering
L^y(T^-_{k},t)=L^y(T^-_k)+mv^z_c(T^-_k)(p^x_{sw}(T^-_{k}-p^x_{st}(T^-_{k}))
\label{eq:L_next_fast}
\end{aligned}
\end{equation}

As a result, the footstep placement equation must be updated to:

\begin{equation}
\begin{aligned}
p^{x,d}_{sw}(T^-_k)=\dfrac{L^{y,d}(T^-_{k+1})}{m(H\omega sinh(\omega T)-v^z_{CoM})cosh(\omega T)}-\\
\frac{(L^y(T^-_k)+mv^z_{CoM}(T^-_k)p^x_{st}(T^-_k))cosh(\omega T)}{m(H\omega sinh(\omega T)-v^z_{CoM})cosh(\omega T)}
\label{eq:L_next_fast}
\end{aligned}
\end{equation}


\subsection{Time Constrained Phase Space Planning}

The model is describe as 
\begin{equation}
\begin{aligned}
\centering
\begin{bmatrix}
\dot{x} \\
\ddot{x} 
\end{bmatrix}
=
\begin{bmatrix}
0 & 1 \\
\frac{g}{H} & 0
\end{bmatrix}
\begin{bmatrix}
x \\
\dot{x}
\end{bmatrix}
\label{eq:LIMP}
\end{aligned}
\end{equation}

From section~\label{X}, we can conclude that the LTL makes decision on the locomotion hyperparameters. There are two modes: mode 1 and mode 2.

Mode 1 is where the LTL select forward angular momentum $L_y$, lateral angular momentum $L_x$ and next step time $T$. This mode emphasis the time constraint over the next step and the robot wants to achieve a desired angular momentum at next keyframe using step time $T$.

In this case, we would use LIPM dynamics to calculate when the next switch happens. The switch time devide the apex-to-apex step into two parts, the first part takes $t_1$ and the second part takes $t_2$.

So we have $t_1+t_2=T$. Also, from the LIPM dynamics, we have the analytical solution of the system state when CoM height is fixed to $H$ and 
\begin{equation}
\begin{aligned}
\centering
\begin{bmatrix}
x(t) \\
\dot{x}(t)
\end{bmatrix}
=
\begin{bmatrix}
(x_0-x_{st})cosh(\omega t) + \frac{\dot{x}_0}{\omega}sinh(\omega t) + x_{st}\\
\omega (x_0-x_{st})sinh(\omega t) + \dot{x}_0cosh(\omega t) 
\end{bmatrix}
\label{eq:LIMP_solution_general}
\end{aligned}
\end{equation}

When the initial state is an apex state $(x(0), \dot{x(0)}) = (0, \dot{x}_0)$.

\begin{equation}
\begin{aligned}
\centering
\begin{bmatrix}
x(t) \\
\dot{x}(t)
\end{bmatrix}
=
\frac{\dot{x}_0}{2\omega}\begin{bmatrix}
e^{\omega t} - e^{-\omega t} \\
\omega e^{\omega t} + \omega e^{-\omega t}
\end{bmatrix}
\label{eq:LIMP_solution_apex}
\end{aligned}
\end{equation}

So from the current apex state $(0, \dot{x}_c)$, we can forward predict the contact switch state to $(x_{switch}^c, \dot{x}_{switch}^c)$. Similarly, we can backward predict the contact switch state $(x_{switch}^n, \dot{x}_{switch}^n)$ from next apex state $(L, \dot{x}_n)$.

\begin{equation}
\begin{cases}
   x_{\rm switch}^c = \frac{\dot{x}_c}{2\omega} (e^{\omega t_1} - e^{-\omega t_1}) \\
   \dot{x}_{\rm switch}^c = \frac{\dot{x}_c}{2} (e^{\omega t_1} + e^{-\omega t_1}) \\
   x_{\rm switch}^n = L-\frac{\dot{x}_n}{2\omega} (e^{\omega t_2} - e^{-\omega t_2}) \\
   \dot{x}_{\rm switch}^n = \frac{\dot{x}_n}{2} (e^{\omega t_2} + e^{-\omega t_2}) 
\end{cases}
\end{equation}

From $t_1 + t_2 = T, \dot{x}_{\rm switch}^c = \dot{x}_{\rm switch}^n$, we can compute 
\begin{equation}
\begin{cases}
   t_1 = \frac{T}{2} + \frac{1}{2\omega} \log(\frac{e^{\omega T}-A}{Ae^{\omega T}-1}) \\
   t_2 = \frac{T}{2} - \frac{1}{2\omega} \log(\frac{e^{\omega T}-A}{Ae^{\omega T}-1})
\end{cases}
\end{equation}
where $A  = \frac{\dot{x}_c}{\dot{x}_n}$.

The step length $L = \frac{\dot{x}_0}{\omega} (sinh(\omega t_1) + sinh(\omega t_2))$ based on analytical solution.

\subsection{Apex Momentum Plannning}
Planning between apex dynamic states aligns with Phase Based Planning. As a result, planning footsteps based on phase space requires a modification of Equation \ref{eq:LIMP_momentum}. 

\begin{equation}
\begin{aligned}
L^y(t_1) &= mHlsinh(l((t_1-t)) x(t) + cosh(l((t_1-t)) L^y(t)\\
L^{yd}(t_2) &= mHlsinh(l((t_2)) p_{st} + cosh(l((t_2)) L^y(t_1)
\end{aligned}
\end{equation}

\subsection{Two-step horizon}
Two-step foot placement calculation is necessary when we adopt apex-to-apex planning.


\subsection{Step Constrained Phase Space Planning}

In mode 2, the LTL select forward angular momentum $L_y$, lateral angular momentum $L_x$ and next step length $L$. This is useful when we need to step on specific foot location, so the foot location constraints are prioritized over step time. 

From this mode, we first use sagittal dynamics to compute the $t_1$ and $t_2$, and then compute step width accordingly. 

From the equation 25, we have the state $x_{switch}^c = x_{switch}^n, \dot{x}_{switch}^c = \dot{x}_{switch}^n$. This gives us the solution of $t_1$ and $t_2$:
\begin{equation}
\begin{cases}
   t_1 = \frac{1}{\omega} \log{\frac{\sqrt{4\dot{x}_c^2\omega^2L^2+(\dot{x}_c^2-\dot{x}_n^2-\omega^2L^2)^2} - (\dot{x}_c^2-\dot{x}_n^2-\omega^2L^2)}{2\omega \dot{x}_c L}} \\
   t_2 = \frac{1}{\omega} \log{\frac{\sqrt{4\dot{x}_c^2\omega^2L^2+(\dot{x}_c^2-\dot{x}_n^2-\omega^2L^2)^2} + (\dot{x}_c^2-\dot{x}_n^2+\omega^2L^2)}{2\omega \dot{x}_n L}}
\end{cases}
\end{equation}

% Different from Mode 1, we cannot using analytical forward and backward prediction. So here we use a numerical forward and backward propogation to compute the t_1 and t_2, until the first and second phase meet each other at contact time. 

Finally, with $t_1$ and $t_2$ solved, we can solve the step width analytically. We want the lateral velocity to be zero at apex state. % distance between the foot and CoM to be a nominal value $\Delta y_2 = 0.13m$ for cassie. 
We define the lateral distance between CoM and the stance foot location as $w(t) = y(t) - y_{st}$.
The equation \ref{eq:LIMP_solution_general} in lateral direction can be represented as:
\begin{equation}
\begin{aligned}
\centering
\begin{bmatrix}
w(t) \\
\dot{w}(t)
\end{bmatrix}
=
\begin{bmatrix}
w(t_0)cosh(\omega t) + \frac{\dot{y}_0}{\omega}sinh(\omega t)\\
\omega w(t_0)sinh(\omega t) + \dot{y}_0cosh(\omega t) 
\end{bmatrix}
\label{eq:LIMP_width_solution}
\end{aligned}
\end{equation}

So the step width $W = w(t_1) + w(t_2) = \\ w_0^c cosh(\omega t_1) + \frac{\dot{y}^c sinh(\omega t_1) + \dot{y}^n sinh(\omega t_2)}{\omega} + \frac{cosh(\omega t_2)}{\omega sinh(\omega t_2)}(w_0^c \omega sinh(\omega t_1) + \dot{y}^c cosh(\omega t_1) - \dot{y}^n cosh(\omega t_2))$, $w_0^c = w^c(t_0)$.

\subsection{Momentum Phase Space Planning (MPSP)}

In this section we describe how the MPSP is able to complete the decision made by LTL layer and compute a consistent trajectory with LIPM. When we replace the CoM velocity with angular momentum in system state, we get a similar analytical solution from the system dynamics (equation~\ref{eq:LIMP_momentum}). 
% This is a uncomplete version
% \begin{equation}
% \begin{aligned}
% \centering
% \begin{bmatrix}
% \dot{x}(t)\\
% \dot{L}(t)
% \end{bmatrix}
% =
% \frac{1}{2}\begin{bmatrix}
% \frac{c_1}{mH\omega}(e^{\omega t} + e^{-\omega t}) + c_2(e^{\omega t} + e^{-\omega t})\\
% c_1(e^{\omega t} - e^{-\omega t}) + c_2\omega m H(e^{\omega t} - e^{-\omega t})
% \end{bmatrix}
% \label{eq:LIMP_solution}
% \end{aligned}
% \end{equation}
% Where $c_1 = L_y^c, c_2 = 0$ when initial apex state is $(0, L_y^c)$. 

\begin{equation}
\begin{aligned}
\centering
\begin{bmatrix}
x(t)\\
L(t)
\end{bmatrix}
=
\begin{bmatrix}
\frac{L_0}{mH\omega}sinh(\omega t) + (x_0 - x_{st})cosh(\omega t)+x_{st}\\
\omega H m (x_0-x_{st})sinh(\omega t) + L_0cosh(\omega t)
\end{bmatrix}
\label{eq:LIMP_solution}
\end{aligned}
\end{equation}

We have mode 1 and mode 2 in mpsp too. Mode 1 is where the LTL select forward angular momentum $L_y$, lateral angular momentum $L_x$ and next step time $T$. 

From the current and next apex state $(0,L_y^c)$, $(L,L_y^n)$. We can get the time solution: 

\begin{equation}
\begin{cases}
   t_1 = \frac{1}{\omega} \log{\frac{\sqrt{4L_y^{c2} m^2H^2\omega^2L^2+(L_y^{c2}-L_y^{n2}-m^2H^2\omega^2L^2)^2} - (L_y^{c2}-L_y^{n2}-m^2H^2\omega^2L^2)}{2\omega L_y^c mH L}} \\
   t_2 = \frac{1}{\omega} \log{\frac{\sqrt{4L_y^{c2} m^2H^2\omega^2L^2+(L_y^{c2}-L_y^{n2}-m^2H^2\omega^2L^2)^2} + (L_y^{c2}-L_y^{n2}+m^2H^2\omega^2L^2)}{2\omega L_y^n mH L}} 
\end{cases}
\end{equation}

% Finally, with $t_1$ and $t_2$ solved, we have the step length and step width solved too. $L = \frac{L_y^c}{mH\omega}sinh(\omega t_1) + \frac{L_y^n}{mH\omega}sinh(\omega t_2)$ and $W = ...$.

Finally, with $t_1$ and $t_2$ solved, we have the step length and step width solved too. $W_x = p^d_{sw} + p_{st}$ and $W_y = ...$.

Mode 2 is where the LTL select forward angular momentum $L_y$, lateral angular momentum $L_x$ and step length $L$. 


\section{Tracking Control}
In this section we examine the tracking controller for cassie used to follow the desired joint commands. We use a passivity-based controller adapted from [] to a floating base model

\begin{equation}
\begin{aligned}
\centering
M(q)\ddot{q}+G(q,\dot{q})=Bu+J_c(q)^T\tau_c+J_{sp}^T\tau_{sp}
\label{eq:dyncnstr}
\end{aligned}
\end{equation}
where $u$ is the motor torques, $\tau_{sp}$ is the spring torques, $\tau_c$ is the contact wrench, $J_s$ is the spring jacobian, and $J_c$ is the contact jacobian. The dynamics of system are represented by joint angle $q$, velocity $\dot{q}$, and accelerations $\ddot{q}$. The coriolis and gravity matrices are represented with $G$ and the mass matrix $M$.

Multiple model simplifications are made to formulate the system's control. A line contact at Cassie's feet during the single support phase do not provide six holonomic constraints and leaves the foot roll as a free degree of freedom (Equation \ref{eq:accel_cntr}). In addition, the springs are assumed to be rigid once firmly in contact (Equation \ref{eq:rigid_cntr}), which provides two constraints per leg. Cumulatively, these simplifications reduce the 20 DoF floating base model to 11 DoF. 

\begin{equation}
\begin{aligned}
\centering
J_s\ddot{q}=0 
\label{eq:rigid_cntr}
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
\centering
J_c(q)\ddot{q}+\dot{J}_c(q)\dot{q}=0 
\label{eq:accel_cntr}
\end{aligned}
\end{equation}

As a result, the full dynamic model for Cassie while in single stance support can be formulated as the following:

\begin{equation}
\begin{aligned}
\centering
\underbrace{
\begin{bmatrix}
M & -J_s^T & -J_c^T \\
J_s & 0 & 0 \\
J_c & 0 & 0
\end{bmatrix}}_{\tilde{M}}
\underbrace{
\begin{bmatrix}
\ddot{q} \\
\tau_{sp} \\
\tau_c
\end{bmatrix}}_{\tilde{f}}
+
\underbrace{
\begin{bmatrix}
G \\
0 \\
\dot{J}_c\dot{q}
\end{bmatrix}}_{\tilde{G}}
=
\underbrace{
\begin{bmatrix}
B \\
0 \\
0
\end{bmatrix}}_{\tilde{B}}
\label{eq:dyn}
\end{aligned}
\end{equation}

The coordinates can be decomposed into both controllable (actuated), $q_a$, and uncontrollable, $q_u$, components $q=[q_a,q_u]^T$. An uncontrolled state vector $\tilde{f}_u=[q_u,\tau_{sp},\tau_c]^T$ can then be used to partition Equation \ref{eq:dyn} into two component equations:
\begin{equation}
\begin{aligned}
    \centering
    \begin{bmatrix}
    \Tilde{M}_{11} & \Tilde{M}_{12} \\
    \Tilde{M}_{21} & \Tilde{M}_{22}
    \end{bmatrix}
    \begin{bmatrix}
    \ddot{q}_a\\
    \tilde{f}_u
    \end{bmatrix}+
    \begin{bmatrix}
    \tilde{G}_1\\
    \tilde{G}_2
    \end{bmatrix}=
    \begin{bmatrix}
    \tilde{B}_1\\
    \tilde{B}_2
    \end{bmatrix}u
    % \def\arraystretch{1.1}
    % \begin{blockarray}{r@{\;}l}
    %     \begin{block}{r@{\;}l\}}
    %     \Tilde{M}_{11}\ddot{q}_a+\tilde{M}_{12}\tilde{f}_u+\tilde{G}_1=\Tilde{B}_1u & \\[\jot]
    %     \Tilde{M}_{21}\ddot{q}_a+\tilde{M}_{22}\tilde{f}_u+\tilde{G}_2=\Tilde{B}_2u & \\[\jot]
    %     \end{block}
    % \end{blockarray}
    % \label{eq:partition}
\end{aligned}
\end{equation}

Solving the above equation, we eliminate the $\tilde{f}_u$ and obtain the following set of partial passive-dynamic equations dictated by the controllable components:

\begin{equation}
\begin{aligned}
\centering
\bar{M}\ddot{q}_a+\Bar{G}=\Bar{B}u
\label{eq:partial_dyn}
\end{aligned}
\end{equation}
where
\begin{equation}
\begin{aligned}
    \bar{M}=\tilde{M}_{11}-\tilde{M}_{12}\tilde{M}_{22}^{-1}\tilde{M}_{21} \\
    \bar{G}=\tilde{G}_{1}-\tilde{M}_{12}\tilde{M}_{22}^{-1}\tilde{G}_{2} \\
    \bar{B}=\tilde{B}_{1}-\tilde{M}_{12}\tilde{M}_{22}^{-1}\tilde{B}_{2} \\
    \label{eq:decompose}
\end{aligned}
\end{equation}

The Passivity-based Controller can then be defined with error dynamics for $y:=q_a-q_r$ such that

\begin{equation}
\begin{aligned}
\Bar{M}\ddot{y}+(\Bar{C}+k_d)\dot{y}+k_py=0 
\label{eq:passivityctrl}
\end{aligned}
\end{equation}
where $\bar{M}$ is the mass matrix and $\bar{C}$ is the Coriolis matrix in $\bar{G}$ such that $\dot{\bar{M}}=\bar{C}+\bar{C}^T$. Reformulating Equation \ref{eq:partial_dyn} with Equation \ref{eq:passivityctrl} provides the following commanded torque law
\begin{equation}
\begin{aligned}
u=\Bar{B}^{-1}(\Bar{M}\ddot{q}_r+\Bar{G})-\Bar{B}^{-1}(k_py+(\Bar{C}+k_d)\dot{y})
\label{eq:passivityctrl}
\end{aligned}
\end{equation}
The resulting passivity-based controlled cancels less of the robot's dynamics, resulting in improved tracking performance over simple joint input-output joint PD implementations [].

\subsection{capture point}

During walking, the robot is encountered a situation where it has to come to a complete stop immediately. This scenario could come from the situation where the robot sees a barrier in the front and need to avoid collision. The planning of such motion is similar to the capture point work \cite{pratt2006capture}. Based on the LIPM, the foot placement to stop a robot is $p_{BFx} = \frac{\dot{x}_f}{\omega}$.
\begin{equation}
\begin{aligned}
\centering
\begin{bmatrix}
x(t) \\
\dot{x}(t)
\end{bmatrix}
=
\begin{bmatrix}
- \frac{\dot{x}_0}{\omega} e^{-\omega t} \\
\dot{x}_0  e^{-\omega t}
\end{bmatrix}
\label{eq:LIMP_solution_apex}
\end{aligned}
\end{equation}
It takes $t2 = \infty$ and $p_{BFy} = \frac{\dot{y}_f}{\omega}$. where $p_{BFx}$ and $p_{BFy}$ represent foot location in CoM frame in sagittal and lateral direction, $\dot{x}_f$ and $\dot{y}_f$ is the velocity at contact time.
